Local Implicit Normalizing Flow for Arbitrary-Scale Image Super-Resolution

Flow-based methods have demonstrated promising results in addressing the ill-posed nature of super-resolution (SR) by learning the distribution of high-resolution (HR) images with the normalizing flow. However, these methods can only perform a predefined fixed-scale SR, limiting their potential in real-world applications. Meanwhile, arbitrary-scale SR has gained more attention and achieved great progress. Nonetheless, previous arbitrary-scale SR methods ignore the ill-posed problem and train the model with per-pixel L1 loss, leading to blurry SR outputs. In this work, we propose "Local Implicit Normalizing Flow" (LINF) as a unified solution to the above problems. LINF models the distribution of texture details under different scaling factors with normalizing flow. Thus, LINF can generate photo-realistic HR images with rich texture details in arbitrary scale factors. We evaluate LINF with extensive experiments and show that LINF achieves the state-of-the-art perceptual quality compared with prior arbitrary-scale SR methods.

==> tables/Table3-5.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\footnotesize
\resizebox{2\columnwidth}{!}{%
    \begin{tabular}{lccc|lcccc|lcccc}
        \hline
        (a) Computation time & LPIPS $\downarrow$ & Time (s)$\downarrow$ & \#Param & (b) Fourier nsemble & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Time (s)$\downarrow$ & (c) Local region size & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Time (s)$\downarrow$ \\
        \hline
        LAR-SR~\cite{larsr} & 0.114 & 14.70 & 62.1M & Local ensemble & \textbf{29.04} & 0.82 & \textbf{0.270} & 2.16 & Pixel-based $\tau$=0 & \textbf{29.04} & 0.82 & 0.271 & 1.44 \\
        SRFlow $\tau=0.9$~\cite{srflow} & 0.121 & 1.43 & 39.5M & Fourier ensemble (-W) & 29.03 & 0.82 & 0.271 & \textbf{1.39} & Pixel-based $\tau$=0.6 & 27.54 & 0.77 & 0.174 & 1.44 \\
        HCFlow++ $\tau=0.9$~\cite{hcflow} & \textbf{0.111} & 1.46 & 23.2M & Fourier ensemble & \textbf{29.04} & 0.82 & \textbf{0.270} & 1.44 & Patch-based $\tau$=0 & 28.85 & 0.82 & 0.273 & 0.33 \\
        Ours $\tau=0.8$ & 0.112 & \textbf{0.54} & \textbf{17.5M} & & & & & & Patch-based $\tau$=0.6 & 27.43 & 0.77 & \textbf{0.158} & 0.33 \\
        \hline
    \end{tabular}
}
\caption{The x4 SR results of different methods and ablation studies on the DIV2K\cite{div2k} validation set. -W refers to removing the amplitude scaling. The time is evaluated on an NVIDIA TITAN X GPU.}
\label{tab:exp:table3-5}
\end{table*}


==> tables/ensemble.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\footnotesize
\resizebox{.8\columnwidth}{!}{%
    \begin{tabular}{l|c|c|c|c}
        \hline
        Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Time (s)$\downarrow$ \\
        \hline
        \hline
        Local ensemble & 29.04 & 0.82 & 0.270 & 2.16 \\
        Fourier ensemble (-W) & 29.03 & 0.82 & 0.271 & 1.39 \\
        Fourier ensemble & 29.04 & 0.82 & 0.270 & 1.44 \\
        \hline
    \end{tabular}
}
\caption{The x4 SR results of different ensemble methods on the DIV2K\cite{div2k} validation set. -W refers to removing the amplitude scaling. The time is evaluated on an NVIDIA TITAN X GPU.}
\label{tab:exp:ensemble}
\end{table}

==> tables/generative_on_arbitrary.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\footnotesize
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c|c|c|c}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{4}{c}{Scale} \\ 
         & \multicolumn{1}{c}{x3} & \multicolumn{1}{c}{x3.25} & \multicolumn{1}{c}{x3.5} & \multicolumn{1}{c}{x3.75} \\ \hline \hline
         
        ESRGAN (+bicubic) \cite{esrgan} & 28.94 / 0.076 & 28.37 / 0.087 & 27.85 / 0.097 & 27.39 / 0.107 \\
        
        RankSRGAN (+bicubic) \cite{ranksrgan} & 28.63 / 0.087 & 28.09 / 0.097 & 27.61 / 0.108 & 27.19 / 0.118 \\
        
        SRFlow (+bicubic) $\tau$ = 0.9 \cite{srflow} & 29.33 / 0.082 & 28.77 / 0.092 & \textbf{28.26} / 0.103 & \textbf{27.77} / 0.113 \\ 
        
        HCFlow (+bicubic) $\tau$ = 0.9 \cite{hcflow} & 28.88 / 0.072 & 28.32 / 0.082 & 27.81 / 0.092 & 27.36 / 0.102 \\
        
        \textbf{Ours} $\tau$ = 0.8 & \textbf{29.44} / \textbf{0.069} & \textbf{28.79} / \textbf{0.080} & 28.24 / \textbf{0.090} & 27.76 / \textbf{0.101}  \\
        \hline
        
       
    \end{tabular}
}
\caption{The arbitrary-scale SR results  (PSNR / LPIPS) evaluated on the DIV2K validation set, where the values of PSNR are evaluated on the RGB space. (+bicubic) means that the model first generates $\times$4 HR image and then down-scale to the specified scale using bicubic interpolation.}
\label{tab:exp:generative_on_arbitrary}
\end{table}

==> tables/notation.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\footnotesize
\setlength{\tabcolsep}{1.5em}
\resizebox{1.8\columnwidth}{!}{%
    \begin{tabular}{c|l}
        \mytoprule
        Symbol & Description  \\
        \mytoprule
        $n$ & Patch size of our LINF model. \\
        $I^{LR}$ & Low Resolution image. \\
        $I^{HR}$ & High Resolution image. \\
        $I^{LR}_{\uparrow}$ & Bilinearly upsampled Low Resolution image. \\
        $I^{HR}_{texture}$ & Texture of High Resolution image, defined as the residual between $I^{HR}$ and $I^{LR}_{\uparrow}$. \\
        $s$ & Upscaling factor. \\
        $m_{i,j}$ & Local texture patch with index $(i, j)$. \\
        $x_{i,j}$ & Coordinate of local texture patch $m_{i,j}$. \\
        \hline
        $f_{\theta}$ & Normalizing Flow model with parameter $\theta$. \\
        $z$ & Latent variable with Gaussian distribution. \\
        $h$ & Intermediate latent variable in the flow transformation. \\
        $\tau$ & Temperature of Gaussian distribution, i.e, variance. \\
        \hline
        $E_{\Psi}$ & Local Texture Estimator with parameter $\Psi$.\\
        $g_{\Phi}$ & Parameter Generator with parameter $\Phi$.\\
        $c$ & Cell size, calculated as $c=2/s$. \\
        $v$ & Feature vector of Low Resolution image. \\
        $\Upsilon$ & The set of four nearest feature vectors given a query coordinate $x_q$. \\
        $w$ & Ensemble weight of bilinear interpolation. \\
        \mytoprule
    \end{tabular}
}
\caption{A list of the symbols used in this paper.}
\label{tab:supp:notation}
\end{table*}

==> tables/patch_size.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\footnotesize
\resizebox{0.8\columnwidth}{!}{%
    \begin{tabular}{l|c|c|c}
        \hline
        Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \hline
        \hline
        n = 1 (pixel) & 27.94 & 0.79 & 0.174 \\
        n = 3 (3$\times$3 patch) & 27.43 & 0.77 & 0.158 \\
        n = 5 (5$\times$5 patch) & 27.41 & 0.77 & 0.153 \\
        \hline
    \end{tabular}
}
\caption{The impact of the local patch size n on different performance metrics. The results are evaluated on the DIV2K validation set with temperature $\tau=0.6$.}
\label{tab:supp:patch_size}
\end{table}

==> tables/pixel_vs_patch.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\footnotesize
\resizebox{.75\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c}
        \hline
        Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Time~(s) \\
        \hline
        \hline
        Pixel-based $\tau$=0 & \textbf{29.04} & 0.82 & 0.271 & \multirow{2}{*}{1.44} \\
        Pixel-based $\tau$=0.6 & 27.54 & 0.77 & 0.174 \\
        \hline
        Patch-based $\tau$=0 & 28.85 & 0.82 & 0.273 & \multirow{2}{*}{0.33} \\
        Patch-based $\tau$=0.6 & 27.43 & 0.77 & \textbf{0.158} \\
        
        \hline
    \end{tabular}
}
\caption{The x4 SR results of the pixel-based and patch-based models on the DIV2K\cite{div2k} validation set. The computation time is evaluated on an NVIDIA TITAN X GPU.}
\label{tab:exp:pixel_vs_patch}
\end{table}
